Three arguable and interrelated concepts: point particle singularity, asymmetric action of EM on quantum wave functions, and the Left out restricted Lorentz gauge from U(1)

We address three issues. i. The point particle assumption, inherent to non-quantum physics, is singular and entails divergent fields and integrals. ii. In quantum physics EM plays an asymmetric roll. It acts on quantum wave fields (wave functions) but the wave fields do not react back. We suggest to promote the one sided action of EM on quantum fields into a mutual action-reaction partnership. By so doing, the quantum wave shares its analyticity with the EM field and removes the later's singularities and divergences. iii) The conventional U(1) symmetry leaves quantum dynamics invariant under a 'general' Lorentz gauge and impose the standard minimal coupling of the quantum wave to the Em 4-vector potential. One, however, has the option to ask for in-variance under the 'restricted' Lorentz gauge. This in turn invites in a coupling to derivatives of the vector potential in addition to the minimal coupling and, so to say, enlarges the U(1) symmetry. We find that the electron exhibits distributed charge- and current- densities. The enlarged symmetry is expected to bring in its own constant of motion. Indeed it does. The anomalous g-factor of the so designed electron emerges, up to order ({\alpha}/{\pi})^2 as the new constant of motion but, without invoking the QED formalism.

==> BibliographyFile.bib.tex <==
@article{aoyama2015tenth,
  title={Tenth-order electron anomalous magnetic moment: Contribution of diagrams without closed lepton loops},
  author={Aoyama, Tatsumi and Hayakawa, Masashi and Kinoshita, Toichiro and Nio, Makiko},
  journal={Physical Review D},
  volume={91},
  number={3},
  pages={033006},
  year={2015},
  publisher={APS}
}
@incollection{pauli1988quantenmechanik,
  title={Zur quantenmechanik des magnetischen elektrons},
  author={Pauli, Wolfgang},
  booktitle={Wolfgang Pauli},
  pages={282--305},
  year={1988},
  publisher={Springer}
}
@article{schwinger1948quantum,
  title={On quantum-electrodynamics and the magnetic moment of the electron},
  author={Schwinger, Julian},
  journal={Physical Review},
  volume={73},
  number={4},
  pages={416},
  year={1948},
  publisher={APS}
}
@article{aoyama2017erratum,
  title={Erratum: Tenth-order electron anomalous magnetic moment: Contribution of diagrams without closed lepton loops [Phys. Rev. D 91, 033006 (2015)]},
  author={Aoyama, Tatsumi and Hayakawa, Masashi and Kinoshita, Toichiro and Nio, Makiko},
  journal={Physical Review D},
  volume={96},
  number={1},
  pages={019901},
  year={2017},
  publisher={APS}
}
@article{born1934foundations,
  title={Foundations of the new field theory},
  author={Born, Max and Infeld, Leopold},
  journal={Proceedings of the Royal Society of London. Series A, Containing Papers of a Mathematical and Physical Character},
  volume={144},
  number={852},
  pages={425--451},
  year={1934},
  publisher={The Royal Society London}
}
@article{lande1941finite,
  title={Finite self-energies in radiation theory. Part II},
  author={Land{\'e}, Alfred and Thomas, Llewellyn H},
  journal={Physical Review},
  volume={60},
  number={7},
  pages={514},
  year={1941},
  publisher={APS}
}
@article{lande1944finite,
  title={Finite self-energies in radiation theory. part III},
  author={Land{\'e}, Alfred and Thomas, Llewellyn H},
  journal={Physical Review},
  volume={65},
  number={5-6},
  pages={175},
  year={1944},
  publisher={APS}
}

@article{petermann1957fourth,
  title={Fourth order magnetic moment of the electron},
  author={Petermann, Andr{\'e}},
  journal={Helvetica Physica Acta (Switzerland)},
  volume={30},
  year={1957},
  publisher={CERN, Inst. for Theoretical Physics, Copenhagen}
}

@article{blinder2003singularity,
  title={Singularity-free electrodynamics for point charges and dipoles: a classical model for electron self-energy and spin},
  author={Blinder, SM},
  journal={European journal of physics},
  volume={24},
  number={3},
  pages={271},
  year={2003},
  publisher={IOP Publishing}
}
@article{quigg2021notes,
  title={Notes on Lepton Gyromagnetic Ratios},
  author={Quigg, Chris},
  journal={arXiv preprint arXiv:2105.07866},
  year={2021}
}

@article{santos2011plasma,
  title={Plasma-like vacuum in Podolsky regularized classical electrodynamics},
  author={Santos, Roberto Baginski B},
  journal={Modern Physics Letters A},
  volume={26},
  number={25},
  pages={1909--1915},
  year={2011},
  publisher={World Scientific}
}
@article{green1947self,
  title={Self-energy and interaction energy in Podolsky's generalized electrodynamics},
  author={Green, Alex ES},
  journal={Physical Review},
  volume={72},
  number={7},
  pages={628},
  year={1947},
  publisher={APS}
}
@article{lazar2020second,
  title={Second gradient electrodynamics: A non-singular relativistic field theory},
  author={Lazar, Markus and Leck, Jakob},
  journal={Annals of Physics},
  volume={423},
  pages={168330},
  year={2020},
  publisher={Elsevier}
}

 @article{santos2011plasma,
  title={Plasma-like vacuum in Podolsky regularized classical electrodynamics},
  author={Santos, Roberto Baginski B},
  journal={Modern Physics Letters A},
  volume={26},
  number={25},
  pages={1909--1915},
  year={2011},
  publisher={World Scientific}
}

@article{podolsky1948228,
  title={228. B. Podolsky and P. Schwed},
  author={Podolsky, B},
  journal={Rev. Mod. Phys},
  volume={20},
  pages={40},
  year={1948}
}

@article{lazar2020second,
  title={Second gradient electrodynamics: A non-singular relativistic field theory},
  author={Lazar, Markus and Leck, Jakob},
  journal={Annals of Physics},
  volume={423},
  pages={168330},
  year={2020},
  publisher={Elsevier}
}

@book{weinberg1972gravitation,
  title={Gravitation and cosmology: principles and applications of the general theory of relativity},
  author={Weinberg, Steven},
  year={1972},
  publisher={Wiley New York}
}

@book{sakurai2006advanced,
  title={Advanced quantum mechanics},
  author={Sakurai, Jun John},
  pages={122--125},
  year={2006},
  publisher={Pearson Education India}
}
@article{schiff1955quantum,
  title={Quantum Mechanics McGraw-Hill},
  author={Schiff, LI},
  journal={New York},
  volume={19752},
  pages={267--280},
  year={1955}
}

@book{einstein2014meaning,
  title={The meaning of relativity: Including the relativistic theory of the non-symmetric field},
  author={Einstein, Albert},
  volume={32},
  year={2014},
  publisher={Princeton University Press}
}
@misc{jackson1999classical,
  title={Classical electrodynamics},
  author={Jackson, John David},
  year={1999},
  publisher={American Association of Physics Teachers}
}
  
@article{aoyama2012complete,
  title={Complete tenth-order QED contribution to the muon g- 2},
  author={Aoyama, Tatsumi and Hayakawa, Masashi and Kinoshita, Toichiro and Nio, Makiko},
  journal={Physical review letters},
  volume={109},
  number={11},
  pages={111808},
  year={2012},
  publisher={APS}
}

@article{bouchendira2011new,
  title={New determination of the fine structure constant and test of the quantum electrodynamics},
  author={Bouchendira, Rym and Clad{\'e}, Pierre and Guellati-Kh{\'e}lifa, Sa{\"\i}da and Nez, Fran{\c{c}}ois and Biraben, Fran{\c{c}}ois},
  journal={Physical Review Letters},
  volume={106},
  number={8},
  pages={080801},
  year={2011},
  publisher={APS}
}

@article{beier2001new,
  title={New determination of the electron’s mass},
  author={Beier, Thomas and H{\"a}ffner, Hartmut and Hermanspahn, Nikolaus and Karshenboim, Savely G and Kluge, H-J{\"u}rgen and Quint, Wolfgang and Stahl, Stefan and Verd{\'u}, Jos{\'e} and Werth, G{\"u}nther},
  journal={Physical review letters},
  volume={88},
  number={1},
  pages={011603},
  year={2001},
  publisher={APS}
}

@article{hanneke2008new,
  title={New measurement of the electron magnetic moment and the fine structure constant},
  author={Hanneke, D and Fogwell, S and Gabrielse, G},
  journal={Physical Review Letters},
  volume={100},
  number={12},
  pages={120801},
  year={2008},
  publisher={APS}
}
@article{ovsiyuk2016spin,
  title={Spin 1/2 Particle with Anomalous Magnetic Moment in a Uniform Magnetic Field},
  author={Ovsiyuk, EM and Kisel, VV and Voynova, Ya A and Veko, OV and Red'kov, VM},
  journal={Nonlinear Phenomena in Complex Systems},
  volume={19},
  number={2},
  pages={153--165},
  year={2016},
  publisher={Белорусский государственный университет}
}
